SciVer: Evaluating Foundation Models for Multimodal Scientific Claim Verification

We introduce SciVer, the first benchmark specifically designed to evaluate the ability of foundation models to verify claims within a multimodal scientific context. SciVer consists of 3,000 expert-annotated examples over 1,113 scientific papers, covering four subsets, each representing a common reasoning type in multimodal scientific claim verification. To enable fine-grained evaluation, each example includes expert-annotated supporting evidence. We assess the performance of 21 state-of-the-art multimodal foundation models, including o4-mini, Gemini-2.5-Flash, Llama-3.2-Vision, and Qwen2.5-VL. Our experiment reveals a substantial performance gap between these models and human experts on SciVer. Through an in-depth analysis of retrieval-augmented generation (RAG), and human-conducted error evaluations, we identify critical limitations in current open-source models, offering key insights to advance models' comprehension and reasoning in multimodal scientific literature tasks.

==> figure_tex/cot_do.tex <==
\begin{figure}[!t]
 \centering
\includegraphics[width=0.95\linewidth]{figures/cot_do.pdf}
 \caption{Comparison of model performance between CoT reasoning and direct prediction on validation set.
 \yilun{TODO}}
 \label{fig:cot_compare}
\end{figure}

==> figure_tex/subject_distribution.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=0.6\linewidth]{figures/subject_distribution.pdf}
\caption{
Distribution of subjects in \ours.
% For each subject, we recruit at least two graduate students with relevant expertise as annotators (detailed in Appendix~\ref{app:annotator}).
}
\label{fig:subject-distribution}
\end{figure}
